Detection of Compromised Smart Grid Devices with Machine Learning and Convolution Techniques

The smart grid concept has transformed the traditional power grid into a massive cyber-physical system that depends on advanced two-way communication infrastructure to integrate a myriad of different smart devices. While the introduction of the cyber component has made the grid much more flexible and efficient with so many smart devices, it also broadened the attack surface of the power grid. Particularly, compromised devices pose a great danger to the healthy operations of the smart-grid. For instance, the attackers can control the devices to change the behaviour of the grid and can impact the measurements. In this paper, to detect such misbehaving malicious smart grid devices, we propose a machine learning and convolution-based classification framework. Our framework specifically utilizes system and library call lists at the kernel level of the operating system on both resource-limited and resource-rich smart grid devices such as RTUs, PLCs, PMUs, and IEDs. Focusing on the types and other valuable features extracted from the system calls, the framework can successfully identify malicious smart-grid devices. In order to test the efficacy of the proposed framework, we built a representative testbed conforming to the IEC-61850 protocol suite and evaluated its performance with different system calls. The proposed framework in different evaluation scenarios yields very high accuracy (avg. 91%) which reveals that the framework is effective to overcome compromised smart grid devices problem.

==> Crafting.tex <==
\section{Evaluating the Detector} \label{sec:craftingdetector}

We now will discuss the specific cases which two call lists appear, and our approach of discriminating between these two when facing specific cases.

\subsection{Control case}

We have applied our prediction model on a state machine where $q_C$ and $q_M$ produces identical call lists. As expected, the algorithm could not identify between original and compromised device cases, and we have obtained an accuracy rating close to random prediction.

\subsection{Case $SD(L_M, L_C) > 0$}

This is the case where the malicious state makes a type of call that is not contained by the regular state. Discrimination is possible by a boolean feature indicating whether a given call has ever made in the system but it is too simple. For the sake of extensibility into other cases, we used a feature column that indicates total number of calls that has been made to that particular system or library function. Figure~\ref{fig:accs} demonstrates perfect results in this case. 

\subsection{Case $SD(L_C, L_M) > 0$}

This case implies there is a type of call made in the regular state that is not made in the malicious state. Presence of a type of call implies the device has been in the regular state, but gives no information whatsoever about operating in the malicious state. Hypothetically considering two lists of call lists that contains the same amount of calls, statistics about individual calls should make it possible to discriminate between these two states, and it should be possible for a learning algorithm to exploit this information. Figure \ref{fig:accs} indicates perfect results again.

Now that we touched the set difference cases, subsequent cases assume $SD(L_C, L_M) = SD(L_M, L_C) = 0$.

\subsection{Case $LD(L_C, L_M) \neq 0$}

Here, it is implied that two call lists contain the same type of calls but differ only in length. Similar to the previous section, individual statistics about calls in respective lists should make discrimination possible. Figure~\ref{fig:accs} again indicates a perfect result.

With that in mind, subsequent cases assume $LD(L_M, L_C) = 0$, in addition to the previous assumption.

\subsection{Case $ED(L_C, L_M) \neq 0$}

In this case, both call lists contain the same type of calls and they are of the same length, but internal distribution of these calls are not the same, e.g. a call list may contain 1 malloc and 4 free, and another may contain 4 free and 1 malloc.  Similar to previous cases, statistics about individual calls used collectively should make discrimination possible. Figure~\ref{fig:accs} indicates perfect results also in this case.

In our next case, in addition to our two assumptions, we additionally assume $ED(L_C, L_M) = 0$.

\subsection{Case $LvD(L_C, L_M) \neq 0$}

This is the most difficult case. Simply put, two system call list does not differ in summarizing statistics such as total number of calls and call density, but they do differ in the order of calls. To achieve this feat, we have developed algorithms \ref{bucket-algo}, \ref{pred-signal-algo} and \ref{reduction-algo} to be used in succession.

The principal idea is to use a machine learning model that predicts the next sequence of call by inspecting the previous list of calls. If the predictions are true, we can infer the call list is exhibiting expected patterns. On the other hand, if the predictions are failing, we infer the call list is exhibiting unexpected patterns, thus conclude malicious activity is present. 

Upon receiving the call list, first step is to \textit{bucket} the new data. Bucketing could be thought as preparing the data to be fed into the model that generates the prediction signal.

After the bucketing procedure, the prepared data is fed into the pattern predictor. Algorithm \ref{pred-signal-algo} describes the computation required to accomplish this operation. Simply put, for each entry resulting in the dataset after bucketing operation, the predictor yields 0 if it was correctly predicted, 1 if the prediction has failed. Algorithm \ref{bucket-algo} describes the computation required for this operation. 

In the last step, the generated signal is reduced to a single integer variable using a cascade of comvolution and max-pooling. The integer value ought to be higher while facing unexpected activity, and lower when facing expected activity. Cascade of convolution and max-pooling idea originates from convolutional neural networks (CNN) \cite{lecun-iscas-10}, where a much more complex architecture involving these techniques are used for image recognition tasks with astounding success \cite{NIPS2012_4824}. 

At this point, it is good to note that our algorithm uses two distinct learning models: one for generating the raw prediction signal, and second one to inspect the data and make a decision whether the data being processed belongs to an authentic or compromised device. The integer value generated as a result of prediction signal, convolution and max-pooling process is fed into the second machine learning model, along with other features.

In this particular case, omitting this feature from the last prediction model yields an accuracy rating close to the accuracy rating of the control case. The value inferred from the algorithm has boosted the accuracy of our model from random chance to $95$ percent, which can be seen in Figure \ref{fig:accs}.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/theoretical-accuracy.png}
    \caption{Accuracy of our model applied individually to each case.}
    \vspace{-0.2in}
    \label{fig:accs}
\end{figure}

\begin{algorithm}
\small
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    \SetKw{KwBy}{by}
    \DontPrintSemicolon
    \caption{Bucketing}
    \label{bucket-algo}

    \Input{system or library call list}
    \Output{bucketed call list}
    
    \Begin{
        {$S_{bucket}$ $\leftarrow$ configure()}\;
        {$S_{window}$ $\leftarrow$ configure()}\;
        {T $\leftarrow$ configure()}\;
        
        \For{$i \leftarrow 1$ \KwTo input.length - $S_{bucket}$}{
            \For{j $\leftarrow$ 1 to $S_{bucket}$ - 1}{
                R[i][j] {$\leftarrow$} input[i + j - 1]\;
            }
            R[i].last {$\leftarrow$} input[i + $S_{bucket}$ - 1] \;
        }
        
        \KwRet{R}\;
    }
    
\end{algorithm}

\begin{algorithm}
\small
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    \SetKw{KwBy}{by}
    \DontPrintSemicolon
    \caption{Constructing Raw Prediction Signal}
    \label{pred-signal-algo}

    \Input{bucketed call list}
    \Output{raw prediction signal}
    
    \Begin{
        {$S_{bucket}$ $\leftarrow$ configure()}\;
        {$S_{window}$ $\leftarrow$ configure()}\;
        {T $\leftarrow$ configure()}\;
        
        \For{$i \leftarrow 1$ \KwTo R.length}{
            $C_{target}$ {$\leftarrow$} R[i].last \;
            $C_{predict}$ {$\leftarrow$} predict(R[i]) \;
            \eIf{ $C_{predict}$ = $C_{target}$}{
                P[i] {$\leftarrow$} 0 \;
            }{
                P[i] {$\leftarrow$} 1 \;
            }
        }
        
        \KwRet{P}\;
    }
\end{algorithm}


\begin{algorithm}
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    \SetKw{KwBy}{by}
    \DontPrintSemicolon
    \caption{Reducing Raw Prediction Signal}
    \label{reduction-algo}

    \Input{raw prediction signal}
    \Output{an integer giving a measure of how far the call list is straying away from ground truth.}
    
    \Begin{

        {$T_C$} {$\leftarrow$} input\;
        \While{$T_C.length < S_{window}$}{
            \For{$i \leftarrow 1$ \KwTo $T_C.length - S_{window}$}{
                $T_A[i]$ $\leftarrow$ sum from $T_C[i]$ to $T_C[i+S_{window}]$\;
            } 
            
            \For{$i \leftarrow$ 1 \KwTo $T_A.length - S_{window}$ \KwBy $S_{window}$}{
                $T_B[i]$ $\leftarrow$ max from $T_A[i]$ to $T_A[i+S_{window}]$\;
            }
            $T_C$ $\leftarrow$ $T_B$\;
        }
        \KwRet $sum(T_C)$
    }

\end{algorithm}

In this particular case, omitting this feature from the last prediction model yields an accuracy rating close to the accuracy rating of the control case. The value inferred from this algorithm has boosted the accuracy of our model from random chance to $95$ percent.


==> TheoreticalTestbed.tex <==
\section{Simulation Based Study} \label{sec:theoretical-testbed}

The state machine which our features are going to be tested is defined in Figure \ref{fig:test-state-machine}.  Definitions concerning the operation of the machine is as follows:

\begin{itemize}
    \item The period between the start and the end of the operation of the machine is called an \textit{experiment}. 
    \item The machine operates on \textit{events}. Given an event, the machine makes a transition to the state concerned, emits a call list, and returns to the idle state.
    \item Total amount of events to be run in an experiment is randomly chosen according to a gaussian distribution of mean of 10000 and standard deviation of 3000 events.
\end{itemize}
    
The machine operates on following principles:
    
\begin{itemize}
    \item The machine starts at $q_I$.
    \item At each turn, the machine transitions to either state $q_C$ or $q_M$, with state transition probabilities $p_C$ and $p_M$. 
    \item At state $q_C$ and $q_M$, the machine outputs a list of pre-determined call list and transitions back into $q_I$.
    \item After the total amount of events are processed, the machine transitions to terminal state $q_T$ and halts without producing any call trace.
\end{itemize}

\begin{figure}
    \centering

    \begin{tikzpicture}[->, shorten >=5pt, node distance=2.5cm, on grid, auto]
        \node[state, initial] (qi) {$q_I$};
        \node[state] (qm) [right =of qi] {$q_M$};
        \node[state] (qc) [above =of qm] {$q_C$};
        \node[state,accepting] (qt) [below =of qm] {$q_T$};
        
    \path   (qi) edge [bend left] node {$e_C$} (qc)
            (qc) edge node {$r$} (qi)
            (qi) edge [bend right] node[below] {$e_M$} (qm)
            (qm) edge node[above] {$r$} (qi)
            (qi) edge node[below] {$e_T$} (qt);
    \end{tikzpicture}

    \caption{State machine of which our tests are modeled.}
    \label{fig:test-state-machine}
\end{figure}

For each case to be mentioned, there will be a total of 60 experiments, 30 of these will have $p_C = 1$ and $p_M = 0$. The data obtained with these parameters are assumed to be genuine devices. Rest 30 experiments will run with the parameters $p_C = 0.99$ and $p_M = 0.01$. In this case, the data obtained are assumed to be coming from a compromised devices. The task, afterwards, is to craft a set of features that could discriminate between these two states linearly. The classifier naturally follows to be a Support Vector Machine (SVM) with a linear kernel.
 
